Aggressive Sampling for Multi-class to Binary Reduction with Applications to Text Classification

We address the problem of multi-class classification in the case where the number of classes is very large. We propose a double sampling strategy on top of a multi-class to binary reduction strategy, which transforms the original multi-class problem into a binary classification problem over pairs of examples. The aim of the sampling strategy is to overcome the curse of long-tailed class distributions exhibited in majority of large-scale multi-class classification problems and to reduce the number of pairs of examples in the expanded data. We show that this strategy does not alter the consistency of the empirical risk minimization principle defined over the double sample reduction. Experiments are carried out on DMOZ and Wikipedia collections with 10,000 to 100,000 classes where we show the efficiency of the proposed approach in terms of training and prediction time, memory consumption, and predictive performance with respect to state-of-the-art approaches.

==> algorithmic_issues.tex <==
\section{{Double-Sampled Multi-class to Binary Reduction} ($\mRb$) Algorithm}
\label{sec:implem}

In this section, we introduce our proposed $\mRb$ algorithm by detailing two key characteristics: (i) an aggressive, doubly sampled, multi-class to binary reduction; and (ii) an efficient prediction method with candidate pre-selection.




==> relatedwork.tex <==
\section{Related Work}
Large-scale multi-class classification or extreme classification considers problems involving extremely large number of classes and has evolved as a popular branch of machine learning. Such problems are prevalent in real world applications such as text, image or video classification. A number of prior works have addressed different aspects of this problem, which we are going to review in this section.

Some of the earlier contributions in this setting are: one-versus-one (\OVO), \OVA ~\cite{Lorena08}. In {\OVO}, a binary problem is created for each pair of classes of the initial problem. So, this leads to $K(K-1)/2$ binary problems, and as many binary classifiers.The predicted class for a new instance is the one that receives majority of the votes. In {\OVA}, $K$
binary problems are created, in each of them one class is seen as the positive class and the others as negative class. Given real-valued predictors $g_1,\ldots,g_K$, the predicted class for an instance $x$ is given by $\arg\max_yg_y(x).$ In large-scale setting, standard approaches such as $\OVA$ and $\OVO$ become computationally intractable for training and prediction both because they require large number of models. Also, they suffer from the popular problem of class imbalance inherent in large-scale multi-class problems. 

Methods using tree-based classifiers have gained popularity in recent times. These methods rely on binary tree structures where each leaf corresponds to a class and inference is performed by traversing the tree from top to bottom, a binary classifier being used at each node to determine the child node to develop. These methods have logarithmic time complexity. Some of the earlier work in this thread include \cite{Beygelzimer09,bengio2010label}. Whereas some of the popular recent logarithmic-time methods are proposed in \cite{choromanska2013extreme,Choromanska14,daume2016logarithmic,prabhu2014fastxml,bhatia2015sparse}. However, its still a challenging task to find a balanced tree structure which can partition the class labels. Even though the above-mentioned methods have proposed several heuristics to address this problem and are able to reduce the complexity of the model to logarithmic time, empirically they do not show good predictive performance especially in large-class scenario. This is caused by the fact that the prediction error made at a top-level cannot be corrected at lower levels also known as the cascading effect.

Ranking approaches to multi-class classification such as popular multi-class SVM of Crammer and Singer (\cite{Crammer:2002}), works of \cite{Weston98,schapire99,cortes2013multi,lapin2015top}, or the constraint classification framework of \cite{Harpeled02} can be seen as a reduction using binary classifications of pairs of classes (given an example), similar to ours. The proposed reduction strategy allows  to obtain new generalization error bounds, and lead to  a different algorithm. These approaches learn one scoring function per class, and thus have similar computational and sample complexities similar to the {\OVA} approach. So, they are not very favourable in large-class scenarios.

Another recent algorithm to address extreme classification is PD-sparse method \cite{yen2016pd}, where authors use sparsity for high-dimensional datasets. However, sparsity is not guaranteed to generate small size models without hurting model accuracy. Also, another algorithm Log-time Log-space (LTLS) \cite{jasinska2016log} claims to perform extreme classification in logarithmic time and space by embedding large classification problems into simple prediction problems and using dynamic programming for inference. Their empirical results show significant improvement in time and space usage. However the classification accuracy is very low for large-class cases .

In our approach we design similarity features between classes and examples allowing to learn a single parameter vector for the whole problem. A similar approach for learning representations of classes was also proposed in \cite{Weston11}. The latter learns a projection of examples and classes into a low dimensional space, which reduces both training and inference time. In contrast to our approach, the aforementioned learns one parameter vector per class, while we use joint features of classes and examples allowing to reduce the number of vector parameters to one. More recently Mineiro and Karampatziakis \cite{Mineiro15} proposed a method for label embedding using matrix decomposition techniques.

In another line of work, \cite{Titsias2016} proposed an approximation for the softmax layer for calculating probabilities of multi-class classification.
Specifically, the author proposes a new bound on the softmax which factorizes the calculations in a product and thus
avoids to evaluate the normalization constant which can become intractable for very large number of classes. In the case of extreme multi-class classification a doubly stochastic approximation scheme is used, without providing any theoretical guarantees, where one randomly selects a number of candidate classes while performing gradient descent. In our proposed method we also introduce a double stochastic procedure as an unbiased empirical risk minimization of the original expected loss.

